Technical Report: Reactive Planning for Mobile Manipulation Tasks in Unexplored Semantic Environments

Complex manipulation tasks, such as rearrangement planning of numerous objects, are combinatorially hard problems. Existing algorithms either do not scale well or assume a great deal of prior knowledge about the environment, and few offer any rigorous guarantees. In this paper, we propose a novel hybrid control architecture for achieving such tasks with mobile manipulators. On the discrete side, we enrich a temporal logic specification with mobile manipulation primitives such as moving to a point, and grasping or moving an object. Such specifications are translated to an automaton representation, which orchestrates the physical grounding of the task to mobility or manipulation controllers. The grounding from the discrete to the continuous reactive controller is online and can respond to the discovery of unknown obstacles or decide to push out of the way movable objects that prohibit task accomplishment. Despite the problem complexity, we prove that, under specific conditions, our architecture enjoys provable completeness on the discrete side, provable termination on the continuous side, and avoids all obstacles in the environment. Simulations illustrate the efficiency of our architecture that can handle tasks of increased complexity while also responding to unknown obstacles or unanticipated adverse configurations.

==> Makefile <==
#
#  Makefile for automating LaTeX related tasks and administrating a 
#  directory of numerous thesis-related files.
#
#  Prepared by Neil C. Miller
#  Modifed by Lord Simon Cuce III
#  May, 1997
#
#  Revision 2.0 5/12/97
#

INCLUDEFILES = 

	FILENAME = body
	ARCHIVE = backup
	PAPERTYPE = a4

.DEFAULT:
	@echo Sorry, that is an undefined target.

help:
	@echo
	@echo Help for make utility:
	@echo
	@echo   make	    - shows this help.
	@echo   make dvi	- executes latex one time.
	@echo   make clean      - removes all backup and output files.
	@echo   make ps	 - executes dvips one time.
	@echo   make bib	- executes bibtex one time.
	@echo   make all	- runs latex several times, bibtex and dvips.
	@echo   make backup     - creates a .tar.gz backup of all files.
	@echo
	@echo Filenames for the main document and backup archive are 
	@echo specified in the Makefile.
	@echo

%:	
	@echo "$@" | latex $(FILENAME) 

dvi:
	@echo $(INCLUDEFILES)  | latex $(FILENAME)

clean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps

realclean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps *.aux *.bbl *.blg *.ilg *.ind *.lof *.log *.lot *.lof *.toc *.loa *~

ps:
	@dvips -G0 -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)
goodps:
	@dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)

pdf:
	dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o tmp.ps $(FILENAME)
	ps2pdf -dCompatibilityLevel=1.4 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=$(PAPERTYPE) tmp.ps $(FILENAME).pdf
	$(RM) -f tmp.ps

bib:
	@bibtex $(FILENAME)

# This doesn't work perfectly.  For example, the changing of a section
# name does not cause a Warning, even though its change will not be 
# reflected in the TOC until the next pass.  So, "all" should be done 
# after "realclean" before final submission.  Possibly a good use for a 
# small perl script which checks to see that the TOC is up-to-date.
all:
	echo '** Running LaTeX **'
	echo $(INCLUDEFILES) | latex $(FILENAME);
	@if ( grep "There were undefined references"        \
			$(FILENAME).log >/dev/null ); then  \
		echo '** Running BibTeX **';                \
		bibtex $(FILENAME);                         \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	fi
	@while ( grep "Rerun to get cross-references"       \
			$(FILENAME).log >/dev/null ); do    \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	done

oldall:
	@latex $(FILENAME)
	@bibtex $(FILENAME)
	@latex $(FILENAME)
	@latex $(FILENAME)

allps: all
	@dvips -G0 -Ppdf -o $(FILENAME).ps $(FILENAME)

backup:
	@$(RM) $(ARCHIVE).tar.gz
	@tar cf $(ARCHIVE).tar *
	@gzip $(ARCHIVE).tar
	@ls -l $(ARCHIVE).tar.gz



==> backup/ltl-planner-full.tex <==
\section{TEMPORAL LOGIC PLANNING}
\label{sec:ltl_planner}
%\robotpositionunicycle(0),\workspace(0)
%%
%
In this Section, we provide an algorithm to decompose global LTL tasks into point-to-point navigation and manipulation tasks. This process occurs offline i.e., before deploying the robot in the unknown environment. Specifically, in Section \ref{sec:nba} we translate the LTL formula into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA). In Section \ref{sec:dist}, we define a distance metric over this automaton that measures how far the robots are from fulfilling the assigned mission. This metric will be used in Section \ref{sec:planning} to guide and adapt planning to the continuously learned environment by generating high-level navigation and manipulation commands (e.g., `go to region $\ell_j$ and grasp object $\movableobjectdilated_i$'). %The detailed construction of this metric is along the lines of the algorithm proposed in [cite ICRA]\footnote{there are some differences because we have atomic propositions based on robot actions; so this needs to be discussed in the final version. Also, here we have a single robot which simplifies the ICRA algorithm}.
%we convert this automaton into a graph structure that captures the NBA transitions that can be enabled if local reachability problems are solved. The conversion process is presented in Appendix A.  Finally

\subsection{From LTL formulas to Automata}\label{sec:nba}

First, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles}. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\delta_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states; (iii) $\delta_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final states. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times \workspace(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\robotpositionunicycle(t)\in\mathbb{R}^{n\times N}$ and the current structure of the environment $\workspace(t)$. An infinite-length discrete plan $\tau=\robotpositionunicycle(0)\robotpositionunicycle(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if it satisfies the accepting condition of the NBA \cite{baier2008principles}. Particularly, if the sequence of observations/symbols in $\sigma=L(\robotpositionunicycle(0), \workspace(0))L(\robotpositionunicycle(1),\workspace(1))\dots$ can generate at least one infinite sequence of NBA states, starting from the initial NBA state, that includes at least one of the final states infinitely often, then we say that $\tau$ satisfies $\phi$. Hereafter, for simplicity we replace $L(\robotpositionunicycle(t),\workspace(t))$ with $L(\robotpositionunicycle(t))$. 

\subsection{Distance Metric Over the NBA}\label{sec:dist}
\textcolor{red}{[some text/definitions may be removed from the final draft]}
In this Section, given a graph constructed using the NBA, we define a function to compute how far an NBA state is from the set of final states.
%
Following a similar analysis as in [?], first we prune the NBA by removing infeasible transitions that can never be enabled as they require the robot to be in more than one region and/or take more that one action simultaneously.  %(ii) we define a distance metric over the pruned automaton that measures how far the robots are from fulfilling the assigned mission. %among all feasible transitions we identify which transitions are decomposable, i.e., they can be enabled if the robot solves reachability-avoidance planning problems. 
Specifically, a symbol $\sigma\in\Sigma:=2^{\mathcal{AP}}$ is \textit{feasible} if and only if $\sigma\not\models b^{\text{inf}}$, where $b^{\text{inf}}$ is a Boolean formula defined as 
%\pi^{a_j(\movableobjectdilated_i,\movableobjectgoal)}
\begin{align}\label{bInfTSi}
b^{\text{inf}}=&[\vee_{\forall {\ell_i}}( \vee_{\forall \ell_e\neq \ell_i}(\pi^{a_j(\cdot,\ell_e)}\wedge\pi^{a_r(\cdot,\ell_i)}))]\nonumber\\
&\bigvee [\vee_{\forall {a}}(\vee_{\forall a'\neq a}(\pi^{a}\wedge\pi^{a'}))].
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{align}
In words, $b^{\text{inf}}$ requires the robot to be either present simultaneously in more than one disjoint region or take more than one action in a given region at the same time.

Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$. This definition relies on the fact that transition from a state $q_B$ to a state $q_B'$ is enabled if a Boolean formula, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, is satisfied. In other words, $q_B'\in\delta(q_B,\sigma)$, i.e., $q_B'$ can be reached from the NBA state $q_B$ under the symbol $\sigma$, if $\sigma$  satisfies $b^{q_B,q_B'}$. An NBA transition from $q_B$ to $q_B'$ is infeasible if there are no feasible symbols that satisfy $b^{q_B,q_B'}$. All infeasible NBA transitions are removed yielding a pruned NBA automaton. All feasible symbols that satisfy $b^{q_B,q_B'}$ are collected in the set $\Sigma^{q_B,q_B'}$. 



%\subsection{remaining text...}
%In this section, given a graph constructed using the pruned automaton, we define a function to compute how far an NBA state is from the set of final states. %so that final states are visited infinitely, i.e., the accepting condition of the NBA is satsified.
%This metric will be used in Section \ref{sec:planning} to guide planning towards NBA states that are closer to the final states so that final states are visited infinitely, i.e., the accepting condition of the NBA is satisfied.
%By construction of the pruned automaton, for every a state $q_B\in\ccalQ_B^{\text{dec}}$ there exists a symbol that if repeated a finite number of times then another state $q_B'\in\ccalQ_B^{\text{dec}}$ can be visited while this symbol allows to remain in $q_B'$. Also, as discussed before, transition from $q_B$ to $q_B'$ will occur while possibly going through intermediate states but self-loops are
%To this end, we first construct a directed graph $\ccalG=\{\ccalV,\ccalE\}$ as follows. First, to take into account the initial robot state in this process, 
To take into account the initial robot state in the construction of the distance metric, in the pruned automaton we introduce an auxiliary state $q_B^{\text{aux}}$ and transitions from $q_B^{\text{aux}}$ to all initial states $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=L(\robotpositionunicycle(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled based on the initial robot configuration. Hereafter, the auxiliary state $q_B^{\text{aux}}$ is considered to be the initial state of the resulting NBA. %This allows us to exclude NBA transitions that can never be enabled due to the initial robot configuration; see e.g., Figure ??.  

Next, we collect all NBA states that can be reached from $q_B^{\text{aux}}$ in a possibly multi-hop fashion, using a finite sequence of feasible symbols, so that once these states are reached, the robot can always remain in them as long as needed using the same symbol that allowed it to reach this state. Formally, let $\ccalD_{q_B^{\text{aux}}}$ be a set that collects all NBA states $q_B$ (i) that have a feasible self-loop, i.e., $\Sigma^{q_B,q_B}\neq\emptyset$ and (ii) for which there exists a finite and feasible word $w$, i.e., a finite sequence of feasible symbols, so that starting from $q_B^{\text{aux}}$ a finite NBA run $\rho_w$ (i.e., a finite sequence of NBA states) is incurred that ends in $q_B$ and activates the self-loop of $q_B$. In math, $\ccalD_{q_B^{\text{aux}}}$ is defined as:
%$\ccalD_{q_B^{\text{aux}}}$ is defined as:
\begin{align}\label{eq:reach}
    \ccalD_{q_B^{\text{aux}}}=&\{q_B\in\ccalQ_B|\\&(\Sigma^{q_B,q_B}\neq\emptyset)\wedge(\exists w~\text{s.t.}~\rho_{w}=q_B^{\text{aux}}\dots \bar{q}_B q_Bq_B)\nonumber\}.
\end{align}
By definition of $q_B^{\text{aux}}$, we have that $q_B^{\text{aux}}\in\ccalD_{q_B^{\text{aux}}}$.

Among all possible pairs of states in $\ccalD_{q_B^{\text{aux}}}$, we examine which transitions, possibly multi-hop, can be enabled using feasible symbols so that once these states are reached the robot can always remain in them forever using the same symbol that allowed it to reach this state. Formally, consider any two states $q_B, q_B'\in\ccalD_{q_B^{\text{aux}}}$ (i) that are connected through a - possibly multi-hop - path in the NBA, and (ii) for which there exists a symbol, denoted by $\sigma^{q_B,q_B'}$, so that if it is repeated a finite number of times starting from $q_B$, the following finite run can be generated: 
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}q_B^{K},
\end{equation}
where $q_B'=q_B^K$, for some finite $K>0$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B'},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robot cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B'$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B'}$ cannot activate this self-loop; and (iii) $\delta_B(q_B',\sigma^{q_B,q_B'},q_B')$ i.e., there is a feasible loop associated with $q_B'$ that is activated by $\sigma^{q_B,q_B'}$. Due to (iii), the robot can remain in $q_B'$ as long as $\sigma^{q_B,q_B'}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs to generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B'$ that require the robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}. Hereafter, we denote the - potentially multi-hop - transition incurred due to the run \eqref{eq:run} by  $\delta_{B}^m(q_B,\cdot,q_B')$.

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
Then, we construct the directed graph $\ccalG=\{\ccalV,\ccalE\}$ where $\ccalV\subseteq\ccalQ_B$ is the set of nodes and $\ccalE\subseteq\ccalV\times\ccalV$ is the set of edges. The set of nodes is defined so that $\ccalV=\ccalD_{q_B^{\text{aux}}}$ and the set of edges is defined so that $(q_B,q_B')\in\ccalE$ if there exists a feasible symbol that incurs the run $\rho_w$ defined in \eqref{eq:run}. 

Given the graph $\ccalG$, we define the following distance metric.

\begin{definition}[Distance Metric]
Let $\ccalG=\{\ccalV,\ccalE\}$ be the directed graph that corresponds to NBA $B$. Then, we define the distance function $d: \ccalV \times \ccalV \rightarrow \mathbb{N}$ as follows
\begin{equation}\label{eq:dist}
d(q_B,q_B')=\left\{
                \begin{array}{ll}
                  |SP_{q_B,q_B'}|, \mbox{if $SP_{q_B,q_B'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
where $SP_{q_B,q_B'}$ denotes the shortest path (in terms of hops) in $\ccalG$ from $q_B$ to $q_B'$ and $|SP_{q_B,q_B'}|$ stands for its cost (number of hops). 
\end{definition}

In words, $d:\ccalV\times\ccalV\rightarrow \mathbb{N}$ returns the minimum number of edges in the graph $\ccalG$ that are required to reach a state $q_B'\in\ccalV$ starting from a state $q_B\in\ccalV$. This metric can be computed using available shortest path algorithms, such the Dijkstra method with worst-case complexity $O(|\ccalE| + |\ccalV|\log|\ccalV|)$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%

%\normalsize
%\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.
%
Next, we define the final/accepting edges in $\ccalG$ as follows.
\begin{definition}[Final/Accepting Edges]\label{def:accEdges}
An edge $(q_B,q_B')\in\ccalE$ is called final or accepting if the corresponding multi-hop NBA transition $\delta_B^\workspace(q_B,\cdot,q_B')$ includes at least one final state $q_F\in\ccalQ_F$.
\end{definition}

Based on the definition of accepting edges, we define the set $\ccalV_F\subseteq \ccalV$ that collects all states $q_B\in\ccalV$ from which an accepting edge originates, i.e.,
\begin{equation}\label{eq:accNode}
    \ccalV_F = \{q_B\in\ccalV~|~\exists~ \text{accepting edge}~(q_B,q_B')\in\ccalE \}.
\end{equation}
By definition of the accepting condition of the NBA, we have that if at least one of the accepting edges is traversed infinitely often, then the corresponding LTL formula is satisfied. %States $q_B\in\ccalQ_B^{\text{dec}}$ for which there are accepting edges $(q_B,q_B')\in\ccalE$ are collected in a set $\ccalQ_F^{\text{dec}}$.%, i.e.,

Similar to \cite{bisoffi2018hybrid}, we define the distance of any state $q_B\in\ccalV$ to the set $\ccalV_F\subseteq \ccalV$ as
\begin{equation}\label{eq:distF}
d_F(q_B,\ccalV_F)=\min_{q_B'\in\ccalV_F}d(q_B,q_B'),
\end{equation}
where $d(q_B,q_B')$ is defined in \eqref{eq:dist} and $\ccalV_F$ is defined in \eqref{eq:accNode}.

\subsection{Online LTL Planning}\label{sec:planning}

In this Section, we present an online temporal logic planning algorithm for robots that operate in unknown environments. The proposed algorithm requires as an input the graph $\ccalG$ defined in Section \ref{sec:dist}. The main idea is that as the robots navigate the unknown environment, they select NBA states that they should visit next so that the distance to the final states, as per \eqref{eq:distF}, decreases over time. 

Let $q_B(t)\in\ccalV$ be the NBA state that the robots have reached after navigating the unknown environment for $t$ time units. At time $t=0$, $q_B(t)$ is selected to be the initial NBA state. Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}\in\ccalV$ that they should reach next to make progress towards accomplishing their task. This state is selected among the neighbors of $q_B(t)$ in the graph $\ccalG$ based on the following two cases.
%
If $q_B(t)\notin \ccalV_F$, where $\ccalV_F$ is defined in \eqref{eq:accNode}, then among all neighboring nodes, we select one that satisfies
%$q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_B^{\text{dec}}$
\begin{equation}\label{eq:minDist}
d_F(q_B^{\text{next}},\ccalV_F) =  d_F(q_B(t),\ccalV_F)-1,  
\end{equation}
i.e., a state that is one hop closer to the set $\ccalV_F$ than $q_B(t)$ is where $d_F$ is defined in \eqref{eq:distF}.  Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)\in\ccalV_F$; controlling the robot to ensure this property will be discussed in Section \ref{sec:reactive_planner}. If $q_B(t)\in\ccalV_F$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.
  
  
Given the selected state $q_B^{\text{next}}$, a feasible symbol is selected that can enable the transition from $q_B(t)$ to $q_B^{\text{next}}$, i.e., can incur the run \eqref{eq:run}. By definition of the run in \eqref{eq:run}, it suffices to select a symbol that satisfies the following Boolean formula:
\begin{equation}\label{eq:b}
   b^{q_B,q_B'}=b^{q_B,q_B^1}\wedge b^{q_B^2,q_B^3}\wedge\dots b^{q_B^{K-1},q_B^{K}}\wedge b^{q_B^{K},q_B^{K}},
\end{equation}
where $q_B^{K} = q_B^{\text{next}}$. In words, the Boolean formula in \eqref{eq:b} is the conjunction of all Boolean formulas $b^{q_B^{k-1},q_B^{k}}$ that need to be satisfied simultaneously to reach $q_B^{\text{next}}=q_B^K$ through a multi-hop path. Once such a symbol is generated, a point-to-point navigation and manipulation command is accordingly generated. For instance, if this symbol is $\pi^{a_j(\movableobjectdilated_i,\movableobjectgoal)}$ then the robot has to go to region $\movableobjectgoal$ and apply action $a_j$ to the movable object $\movableobjectdilated_i$. The online implementation of such action is discussed in Section \ref{sec:reactive_planner}. %By definition of \eqref{eq:b}, if there exists a feasible symbol $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$ then the finite word generated by repeating $K+1$ times the symbol $\sigma^{q_B,q_B'}$ can yield the run in \eqref{eq:run}.

[+add a few words about completeness of this method+]



%Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}\in\ccalV$ that they should reach next to make progress towards accomplishing their task [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. This state is selected among the neighbors of $q_B(t)$ in the graph $\ccalG$ based on the following two cases.
%
%If $q_B(t)\notin \ccalV_F$, where $\ccalV_F$ is defined in \eqref{eq:accNode}, then among all neighboring nodes, we select one that satisfies
%\begin{equation}\label{eq:minDist}
%d_F(q_B^{\text{next}},\ccalV_F) =  d_F(q_B(t),\ccalV_F)-1,  
%\end{equation}
%i.e., a state that is one hop closer to the set $\ccalV_F$ than $q_B(t)$ is where $d_F$ is defined in \eqref{eq:distF}.  Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)\in\ccalV_F$; design of robot paths to ensure this property will be discussed next. If $q_B(t)\in\ccalV_F$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.

%Recall that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable by construction of $\ccalG$. As a result, to reach $q_B^{\text{next}}$ the robots need to eventually generate a symbol from the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$; this symbol can be selected randomly. By construction of the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, we have that once the robots reach $q_B^{\text{next}}$ they will be able to stay in this state as long as they keep generating this symbol; see \eqref{eq:b} in the Appendix \ref{appA}. With slight abuse of notation, we denote the selected symbol by $\sigma^{\text{next}}$ [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. Also, for simplicity of notation we replace $b^{q_B(t),q_B^{\text{next}}}$ with with $b^{\text{next}}$. %and $b^{q_B(t),q_B(t)}$ with $b^{\text{next}}$ and $b^{\text{inv}}$. The same simplification extends to all notation with the same superscripts.
